InspectJS: Leveraging Code Similarity and User-Feedback for Effective Taint Specification Inference for JavaScript

Static analysis has established itself as a weapon of choice for detecting security vulnerabilities. Taint analysis in particular is a very general and powerful technique, where security policies are expressed in terms of forbidden flows, either from untrusted input sources to sensitive sinks (in integrity policies) or from sensitive sources to untrusted sinks (in confidentiality policies). The appeal of this approach is that the taint-tracking mechanism has to be implemented only once, and can then be parameterized with different taint specifications (that is, sets of sources and sinks, as well as any sanitizers that render otherwise problematic flows innocuous) to detect many different kinds of vulnerabilities. But while techniques for implementing scalable inter-procedural static taint tracking are fairly well established, crafting taint specifications is still more of an art than a science, and in practice tends to involve a lot of manual effort. Past work has focussed on automated techniques for inferring taint specifications for libraries either from their implementation or from the way they tend to be used in client code. Among the latter, machine learning-based approaches have shown great promise. In this work we present our experience combining an existing machine-learning approach to mining sink specifications for JavaScript libraries with manual taint modelling in the context of GitHub's CodeQL analysis framework. We show that the machine-learning component can successfully infer many new taint sinks that either are not part of the manual modelling or are not detected due to analysis incompleteness. Moreover, we present techniques for organizing sink predictions using automated ranking and code-similarity metrics that allow an analysis engineer to efficiently sift through large numbers of predictions to identify true positives.

==> implementation.tex <==
\section{Implementation Details}
\dg{We may include this details in other sections, or remove them as some of them are not very relevant}



==> methodology.tex <==
\section{Methodology}
\subsection{Selection of query-specific JavaScript Libraries}
\TBD{how do we select projects to use with \tool{}?}

\subsection{Evaluating \tool{} using Old Version of CodeQL Query}
Manually evaluating the sinks predicted by \tool{} is
labor-intensive. Hence, we use an alternative strategy to evaluate
\tool{}'s performance. For each given query, we obtain an older
version of the CodeQL library ($V_\text{old}$). We use $V_\text{old}$
to extract source, sanitizer, and sink events from the programs in our
dataset. We add these as known events in \tool{} and predict new
(unknown) sinks and boost the query. We use the boosted query on a set
of test projects to generate alerts. We then compare them against the
alerts generated by the latest version of the query in CodeQL
($V_0$). Since, $V_0$ contains the new sinks and models added by GitHub
engineers since $V_\text{old}$, we use it as a ``ground truth'' for
evaluating \tool{}'s predictions. We compute the precision and recall
of \tool{} using following equations:

\begin{equation}
  \text{Precision} = \frac{|(\text{Sinks}(\text{\tool{}}(V_\text{old})) -
    \text{Sinks}(V_\text{old})) \cap \text{Sinks}(V_0) |}{|\text{Sinks}(\text{\tool{}}(V_\text{old})) - \text{Sinks}(V_\text{old})|}
\end{equation}

\begin{equation}
  \text{Recall} = \frac{|(\text{Sinks}(\text{\tool{}}(V_\text{old})) -
    \text{Sinks}(V_\text{old})) \cap \text{Sinks}(V_0) |}{|\text{Sinks}(V_0) - \text{Sinks}(V_\text{old})|}
\end{equation}

where $\textit{Sinks}$ is a predicate which takes a query/spec as input
and returns the set of sinks extracted using it from a set of test
projects (omitted here for simplicity). 

\NA{This evaluation method provides an under-approximation of
  \tool{}'s actual performance since the false positives predicted by
  \tool{} can potentially belong to a different query. However, we use
  this method as way to quickly evaluate and tune \tool{}'s
  performance instead of manually evaluating the predictions which is
  much more time-consuming and laborious.}

\TBD{should this be sinks or alerts? please replace accordingly}

\subsection{Evaluating \tool{} using Latest Version of CodeQL Query}
\TBD{not clear to me if we are doing this?}
\TBD{is this what we are doing with 90/10 split?}



\subsection{Predicting Alerts}
\TBD{what metrics do we use here?}



==> oldapproach.tex <==
\section{(Old) Technical Approach}
Our approach combines techniques from program analysis, constraint solving and machine learning. 
In Figure~\ref{fig:architecture} we show how we  integrate these elements. 

Given a set of training projects $T$ and some initial knowledge encoded in a security query $Q$ we use \tool{}, our customization of Seldon for javascript, to produce a set of sink predictions $RS$ can be used either to help security engineers to find new sinks when modeling libraries or to automatically improve the existing query to find new alerts.  
%\tool{} uses a taint tracker to produces the set of candidates triples $(source, sanitizer, sink)$ and the constraint solver to produce the 

%% \begin{figure*}
%% 	\includegraphics[scale=0.4]{figures/system}
%% 	\caption{\tool{}: System Overview}\label{fig:Architecture}
%% \end{figure*}

In Algorithm~\ref{alg:main} we show the basic steps to produce the sinks predictions. 
The approach heavily relies on \tool{} which is based on Seldon. 
In section~\ref{sec:TSM} we explain the customization we applied to Seldon to handle javascript programs and to work with CodeQL queries.
Given a query $Q$ and set training projects $T$ \tool{} produces a $sinkSpect  = \in Nodes \times R$ a set of pairs of representations together with a score computed by the constraint solver.
In addition to the sinks specification, \tool{} produces a boosted query $QB$ which is essentially the original query $Q$ extended with the sink specification. 

With $sinkSpect$ and  an evaluation set $E$ the line 4 produces a sink prediction  $PS$ which is a set of program nodes from the training set of projects, which representation matches one of the sink spec. We use the score computed by \tool{} as the initial score for the predictions. 

In line 5 the function $RankPredictions$ defined in Algorithm~\ref{alg:rank}
 combines  the \tool{} score of each prediction with a metric based on the code similarity of the sink prediction with a set of known sinks. 
 
%% \begin{algorithm}
%% 	\caption{Producing and fine tuning of sink predictions}\label{alg:main}
%%     \begin{algorithmic}[1]
%%     \State \textbf{Inputs}: query $Q$, training set $T$, eval set $E$, know sinks $KS$ and its embeddings  $SE$, $FE$	
%% 	\State \textbf{Outputs}: $RS$ ranked sink predictions. 
%% 	\State $(sinkSpec, BQ ) = TSM(Q, T)$
%% 	\State $PS = \{ (s, score)   | s \in p,  p \in E,  (repr(s), score) \in sinkSpec \}$
%% 	\State  $RS = RankPredictions(PS, KS, SE, FE)$
%%     \end{algorithmic}
%% \end{algorithm}



\begin{algorithm}
	\caption{Rank prediction using  known sinks} \label{alg:rank}
	\begin{algorithmic}[1]
		\State \textbf{Inputs}: embeddings for known sinks $SE$, $FE$, known sinks $KS$ predicted sinks $PS$  	
		\State \textbf{Outputs}: ranked predicted sinks $RS$. 
		\State \textbf{Function} $RankPredictions(PS, KS, SE, FE)$
		\State $RPE = \{\}$ 
		\For{sink $s \in PS$}
		\State $(stmCode, funcCode)$ = getEnclonsingCode($s$)
		\State $stmEmb $= embedding($stmCode$)
		\State $funcEmb$= embedding($funcCode$)
		\State $maxStm maxFunc$ = 0 
		\For{sink $s'$ in $\{KS | repr(s') = repr(s) \}$}
			\State $stmEmb'$= $SE(repr(s'), s')$
			\State $funcEmb'$= $SF(repr(s'), s')$
			\State $stmSimil$ = cosineSimilarity($stmEmb$, $stmEmb'$)
			\State $funcSimil$ = cosineSimilarity($funcEmb$, $funcEmb'$)
			\State $maxStm$ = $max(maxStm, stmSimil)$
			\State $maxFunc$ = $max(maxFunc, FuncSimil)$
		\EndFor
		\State $RS$ = $RS \cup (s, (score(s) + (maxStm + maxFunc)/2)/2)$
		\EndFor
		\State return $RS$
	\end{algorithmic}
\end{algorithm}


%We show how we rely on \tool{} to produce sink candidates. 
%
%\subsection{Predicting sinks}
%We use the \tool{} spec (generated with a training set) to produce a set
%of sink candidates for an evaluation set.
%
%The \tool{} spec is a set of tuples (representation, score). We produces a
%set of predictions consisting on a set of (sink location, score).
%$Sinks = \cup_{p \in evalSet} \{ {snk, score} | (repr(snk), score) \in
%\tool{} \wedge snk \in p\}$

\dg{We can add examples of the TSM specs} 

\subsection{Ranking predictions}\label{sec:rank}
\tool{} assigns scores to representations. Each program node 
matching that representation would have the same score regardless on the context of use of that candidate.
In particular, it assigns  the maximum score to all sinks whose representation match
the representation of some known sink. 
Since representations are in general quite coarse (i.e., many different sinks from several projects
have the same representation) it may lead to a great number of false
positives.  
One way to deal with that issue is making representation
fine grainier, but in practice we notice that the effect is having much more representations (i.e., less common representations among different projects) which does not lead to more precision and seriously impact in the scalability of \tool{}, in particular the model construction and constraint solving phase.

As an alternative (and orthogonal) approach, we decided to rely on
similarity metrics to improve the scoring.  The intuition is that a
sink candidate that is somehow similar in term of code to other sinks
that are labelled as true positive (known sinks) is more likely to be
a true sink than other that is not similar to some existing true
sinks. 

The approach is shown in Algorithm~\ref{alg:rank}. 
Given a set of known sinks $KS$ for a set of frequently used queries and a set of projects, 
we produce two embeddings: i) the enclosing
statement of the true sink and ii) the enclosing function.

Then, given a sink candidate we compute its similarity against all the
known sinks. This is done by obtaining the embedding of the sink
candidate and comparing it with the set of precomputed embeddings of the
known sink. 
To get the  similarity between two code snippets we compute the cosine similarity  of  embeddings\footnote{Actually we can compare one code snippet against set of codes and produces a vector of scores.}. 
We keep the similarity score of  the most similar known sink\footnote{For the performance sake we only compare known sinks with the same representation,}).
We apply this approach for the candidate sink enclosing statement and
enclosing function. The final score is the average between this two
scores and the \tool{} score.

%We apply this approach to all predicted sinks, reordering the
%prediction according to the new combined score.

\subsubsection{Computing similarity using embeddings}
\begin{algorithm}
	\caption{Producing embeddings for known sinks}\label{alg:embKS}
	\begin{algorithmic}[1]
		\State \textbf{Inputs}: set of interesting queries $Qs$, training set $T$. 	
		\State \textbf{Outputs}: $SE$, $FE$, embeddings for enclosing statements and enclosing functions for each know sink, grouped by representation. 
		\State $SE = \{\}$ , $FE = \{\}$ 
		\State $ks$ = queryKnownSinks$(Qs,T)$
		\For{knowSink $s \in ks$}
		\State $(stmCode, funcCode)$ = getEnconsingCode($s$)
		\State $stmEmb $= embedding($stmCode$)
		\State $funcEmb$= embedding($funcCode$)
		\State $SE$ = $SE(reprs(s)) \cup s \mapsto  stmEmb$
		\State $SF$ = $SF(reprs(s)) \cup s \mapsto  funcEmb$
		\EndFor
		\State  
	\end{algorithmic}
\end{algorithm}

To compute embeddings we rely on \texttt{CodeBert}~\cite{feng2020codebert}. 
In particular, we use a pre-trained model for clone detection\footnote{\url{https://github.com/microsoft/CodeBERT/tree/master/GraphCodeBERT/clonedetection}.}. 

\dg{Implementation detail, move to another section}
Even though \texttt{CodeBert}  is a framework that is designed to use fine tuned models based on training sets, it is worth noticing that we do not fine tune the model with examples of clones for javascript, we simply rely on vanilla \texttt{CodeBert} to compute embeddings. This is because we couldn't find a labeled set of javascript code with clones. 

In Algorithm~\ref{alg:embKS} we sketch the approach for precomputing embeddings for known sinks.
Given a set of relevant queires $Qs$ and a set of  training project s $T$  we compute embeddings for code snippets of set sinks candidates  grouped by representation.
Essentially, giveb a known sink we get the code for the enclosing statement and enclosing functions use the function $embedding$ to produce an embedding with \text{CodeBert}. 
This comprises the tokenization of the code, invoke the pre trained model produce the encodings, and apply a fixed mean polling to reduce their sizes. 

\dg{implementation details, maybe not relevant}
We save the embeddings for later use. 
For instance, if a representation contains 100 sinks, we produce embeddings for the code snippets of their enclosing statements (resp enclosing functions) and save in a file corresponding to that represenation.
In order to reduce the memory consumption, we split the set of code snippets (and its corresponding embeddings) in chunks. These chunks can me adapted to fit the memory requirements. For instance if a represenation has 100 sinks but the machine cannot handle 10 embeddings  in memory we produce 10 files, one for each chunk with 10 embeddings. 


\subsection{Finding similar examples}
Given a set of sink predictions   we want to quickly find the set of sinks (in the same of predictions) that are similar.  

In Algorithm~\ref{alg:similarSinks} we show how we use embeddings , in a similar fashion to the one explained  in the previous section, to get a set of similar candidates. 
Given a set of predictions $PS$,   the  precomputed embedding for the enclosing statement $PSE$ and the enclosing function $FSE$ of each sink in $PS$ and a candidate $s$ we use $PSE$ and $FSE$ for quickly retrive the embeddings of $s$ and the other candidates and include the sink candidates which cosine similarity values is above a predefined threshold. 


To precompute the embeddings we use a similar approach we used for the known sinks. This is shown in Algorithm~\ref{alg:embPredictions}.

\begin{algorithm}
	\caption{Compute similar sinks}\label{alg:similarSinks}
	\begin{algorithmic}[1]
		\State \textbf{Inputs}: predicted sinks $PS$,$ PSE$, $PFE$  embeddings for predicted sinks, sink $s$ 
		\State \textbf{Outputs}: similar sinks $S$. 
		\State \textbf{Function} $GetSimilarSinks(s, PSE, PFE)$
		\State $S = \{\}$ 
		\State $stmEmb$= $PSE(s)$
		\State $funcEmb$= $PSF(s)$		
		\For{sink $s'  \in dom(PS)$}
		\State $stmEmb'$= $PSE(s')$
		\State $funcEmb'$= $PSF(s')$		
		\State $stmSimil$ = cosineSimilarity($stmEmb$, $stmEmb'$)
		\State $funcSimil$ = cosineSimilarity($funcEmb$, $funcEmb'$)
		\If{$stmSimil + funcSimil/2 > treshold$}
		\State $S$ = $S \cup s'$			
		\EndIf
		\EndFor
		\State return $RS$
	\end{algorithmic}
\end{algorithm}


\subsubsection{Computing similarity of predicted sinks}

\begin{algorithm}
	\caption{Producing embeddings for predicted sinks}\label{alg:embPredictions}
	\begin{algorithmic}[1]
		\State \textbf{Inputs}: $PS$ set of predicted sinks, $T$ training projects. 	
		\State \textbf{Outputs}: $PSE$, $PFE$, embeddings for enclosing statements and enclosing functions for each predicted sink. 
		\State $PSE = \{\}$ , $PFE = \{\}$ 
		\For{sink$s \in PS$}
		\State $(stmCode, funcCode)$ = getEnconsingCode($s$)
		\State $stmEmb $= embedding($stmCode$)
		\State $funcEmb$= embedding($funcCode$)
		\State $PSE$ = $PSE \cup   s \mapsto stmEmb$
		\State $PSF$ = $PSF \cup   s \mapsto funcEmb$
		\EndFor
		\State  
	\end{algorithmic}
\end{algorithm}


\subsection{Putting all together in the UX}



==> oldseldon.tex <==
\Comment{
\subsubsection{Mining flow triples}
The first step of our approach is to mine flow triples of the
form $\langle\mathit{src}, \mathit{san}, \mathit{snk}\rangle$ such that taint
may propagate from $\mathit{src}$ to $\mathit{san}$ and from there to
$\mathit{snk}$. The intuition is that $\mathit{src}$ is a candidate for a sink,
$\mathit{san}$ a candidate for a sanitizer and $\mathit{snk}$ a candidate for a
sink.
Seldon uses a custom program representation referred to as a propagation graph
combined with a points-to analysis as the basis for mining flow triples. 
}

\Comment{
\subsubsection{Generating and Solving Constraint System}
Given the set of events $E$ and set of triples $T$ obtained from the
propagation graphs of the input programs, we build a set of
\emph{information flow constraints}.

\mypara{Variables for Constraint System} For every event $e$ in $E$,
we instantiate three variables: $n^{\textit{src}}$,
$n^{\textit{san}}$, and $n^{\textit{snk}}$, where $n=\texttt{Repr}(e)$
denotes the unique representation of $e$. Each variable
$n^{\textit{src}}, n^{\textit{san}}, n^{\textit{snk}} \in [0,1]$
denotes the likelihood of $n$ being either a source, sanitizer, or
sink. Next we describe how we build the constraints for these
variables.

\mypara{Constraints for variables} Since we want to interpret every
variable as a probability, we add the following constraint for each
variable:
\begin{equation}
	\label{eq:var}
	0 \le n^t \le 1, t \in \{\textit{src}, \textit{san}, \textit{snk}\}
\end{equation}

\mypara{Constraints from known events} Since we start with a small set
of known source, sink, and santizer events, we set the corresponding
variables for their representations accordingly. For instance, for an
event that we know is a sink, we set:
\begin{equation}\label{eq:known}
	\nver{n}{snk}=1, \nver{n}{src}=0, \text{ and } \nver{n}{san}=0
\end{equation}

\mypara{Constraints from triples} We encode our intuitions of
information flow as linear constraints:
\begin{enumerate}
	\item For every sanitizer event $\ever{e}{san}$ that flows into a
	potential sink $\ever{e}{snk}$, the sum of all source candidates
	that flows into the sanitizer must be at least the sum of scores of
	$\ever{e}{san}$ and $\ever{e}{snk}$:
	\begin{equation}    \label{eq:cons1}
		\nver{(\ever{n}{san})}{san} + \nver{(\ever{n}{snk})}{snk} \le
		\mathlarger{\sum}_{i=1}^{k}{\nver{(\ever{n}{i})}{src}} + C
	\end{equation}
	\item For every source $\ever{e}{src}$ that flows into a sanitizer
	$\ever{e}{san}$, the sum of the scores of sinks that the sanitizer
	flows into must be at least the sum of scores of $\ever{e}{src}$
	and $\ever{e}{san}$:
	\begin{equation}    \label{eq:cons2}
		\nver{(\ever{n}{src})}{src} + \nver{(\ever{n}{san})}{san} \le
		\mathlarger{\sum}_{i=1}^{k}{\nver{(\ever{n}{i})}{snk}} + C
	\end{equation}
	\item Analogously, for a source that flows into a sink, we add the
	following constraint:
	\begin{equation}    \label{eq:cons3}
		\nver{(\ever{n}{src})}{src} + \nver{(\ever{n}{snk})}{snk} \le    
		\mathlarger{\sum}_{i=1}^{k}{\nver{(\ever{n}{i})}{san}} + C
	\end{equation}  
\end{enumerate}

Here, $C$ is a fixed constant. Setting $C$ to less than 1 allows us to
relax the constraints when the variables on the left-hand side have
scores of less than 1. \NA{Similar to Seldon~\cite{seldon}, we use
	$C=0.75$.}

We also add another variable $\epsilon$ in
equations~(\ref{eq:cons1},\ref{eq:cons2},\ref{eq:cons3}) which allows
us to further relax the constraints.

\ms{I don't think we actually do what's described in the next paragraph; we use canonical representations instead. Diego?}
\mypara{Handling different event representations} Each event can have
different representations ranging from a the full representation which
identifies the particular API from a library to a coarse one which
only uses the API name. Using the full representation has the risk of
being too specific to the particular API and potentially missing
similar APIs from other libraries, whereas the coarse representation
may be too general and select too many events, many of which may be
false positives.

To account for this, we replace the variables for each event
representation by an average of all its representations:

\begin{equation}  \label{eq:boff}
	\nver{n}{t} = \frac{1}{|\texttt{Reprs(e)}|}
	\mathlarger{\sum}_{r\in\texttt{Reprs(e)}} \nver{(n_r)}{t}, 
	t \in \{\textit{src}, \textit{san}, \textit{snk}\}  
\end{equation}


\mypara{Relaxing flow constraints} Our constraint system contains
variable constraints (Equation~\ref{eq:var}), constraints for known
variables (Equation~\ref{eq:known}), and flow constraints
(Eq~\ref{eq:cons1},\ref{eq:cons2},\ref{eq:cons3}). We consider the
variable and known constraints as hard constraints. We consider the
flow constraints as \emph{soft} constraints since the programs in our
dataset may not respect our intuitions about information flow. Hence,
we add a relaxation variable $\epsilon_i$ for each flow
constraint. More specifically, we transform each flow constraint of
the form: $L_i \le R_i$ to $L_i \le R_i + \epsilon_i$.o

\mypara{Objective function} We build the final objective function for
minimization using a constraint solver:

\begin{equation}
	\mathlarger{\sum}_{i=1}^{M} \text{max}(\epsilon_{i}, 0) +
	\lambda.\mathlarger{\sum}_{{n}_r} (\nver{(n_r)}{src} +
	\nver{(n_r)}{san} + \nver{(n_r)}{snk})
\end{equation}

subject to constraints Eq. \ref{eq:var} and Eq. \ref{eq:known}.

where $M$ is the number of flow constraints, $\lambda$ is a
regularization constant which penalizes solutions which classifies
many nodes as sources, sinks, or sanitizers. In our evaluation we
\NA{used $\lambda=0.1$}.
}

%% In this section we introduce Seldon~\cite{}, the technique to infer
%% taint specifications we used for our approach, and the customizations
%% and design decisions made to support the analyze large javascript
%% projects within in GitHub reposotiries.


\subsection{Adapting Seldon for JavaScript}
\label{sec:TSM}

\begin{figure*}
	\includegraphics[width=1\textwidth]{figures/TSM}
	\caption{\tool{}} \label{fig:TSM}       
\end{figure*}


\begin{itemize}
	\item Modular approach
	\item Representations for JavaScript elemtens (e.g., spliting parameters)
	\item Canonical reps vs detailed reps
	\item Propagation Graph
	\item Use of queries for known sources, sinks, sanitizers. 
	\item use of CodeQL
	\item Filters using adbuction?
\end{itemize}

In Figure~\ref{figures:TSM} we show the architecture of our implementation of the Seldon approach. 
We designed and implemented the components as described in the paper~\cite{seldon}.

The main differences with the original approach is the use of existing queries for computing the known sources, sanitizers and sinks, the of the CodeQL build in taint tracker for getting the candidates triples and two important measures to make the approach scale to huge projects: infer result for each project individually and the compose and reduce the number of representations. In this section we briefly discuss these adaptations.


\mypara{Finding triples}
Seldon uses a custom program representation referred to as a propagation graph combined with a points-to analysis as the basis for mining flow triples. 
We experimented with a similar approach for JavaScript but ran into  several issues, in particular we suffer from recall and precision since the simple alias analysis lead of many spurious aliases but also could not handle many models of libraries implemented in CodeQL which leads to loss on recall as well. In addition the modeling of the propagation graph on CodeQL did not scale well. It either explode with big projects or produces too many triples that cannot be handled by the constraint system. 

Instead, we make use of the standard inter-procedural taint-tracking
implementation shipping with the CodeQL libraries for JavaScript, which is also used by the CodeQL security queries.

Like many other static analyses, CodeQL ignores third-party libraries, making no attempt at analyzing their source code but relying on hand-crafted models to supply the relevant details about the library. 
In particular, this means that if there is flow from a source to a sink, but it passes through a library function for which CodeQL does not have a model, then this flow will not be detected. 
In essence, CodeQL assumes that taint never propagates through unknown functions.

For mining flow triples, we choose the opposite extreme, customizing the CodeQL analysis to instead assume that every unknown function propagates taint from its arguments to its result. 
Similarly, while CodeQL carefully tracks taint through individual properties of objects, our mining analysis assumes that as soon as a
property is tainted the whole object is tainted.

\dg{Warning: we are producing the TSM specs in a per project basis ad the computing the avg}
This can result in lots of false flows, so one would not want to use this kind of analysis for detecting security vulnerabilities. For our purposes, on the other hand, it works well, since we aggregate flow triples across many different code bases, so noise from false flows is likely to be averaged out.


\mypara{Handling scalability} 
We wanted to be able to handle really big projects. Thus, we need to make the analysis scalable. So we apply to important decisions: make the analysis more compositional and reduce the number of representations.

Seldon produces a global propagation graph by composing individual propagation graphs of each project. The constraint system is build out of the representations of all projects together. 
We experienced that in many cases the constraint solver blew up due to the excessive memory consumption. So, we decided to produced models for individual project, produce the scores and the combine them by averaging the scores of nodes with the same representation among several projects . This approach together with the reduction of representations (see below) greatly improved the scalability by the cost of losing some precision.

In order to compare and correlate flow triples mined from
different code bases, we need to represent them in a code base-independent way.
Like Seldon, we use partial access paths in the style of
\textsc{NoRegrets}~\cite{noregrets} for this purpose. 
For instance in Figure~\ref{fig:repr} we show some potential representation for a candidate sink. 

\begin{figure}
	\caption{A sink candidate and its potential representations}
	\begin{lstlisting}[language=JavaScript]
		User.find({username: { $regex } searchUser , $options})
	\end{lstlisting}
	
	\begin{verbatim}
		(member $regex (member username (parameter 0 (member find *))))
		(member $regex (member username (parameter 0 (member find *))))
		(member $regex (member * (parameter 0 (member find *))))
		(member * (member username (parameter 0 (member find *))))
		(member * (member * (parameter 0 (member find *))))
		(member * (member * (parameter *)))
		(member * (member username *))
	\end{verbatim}
	\caption{Possible representations for a sink candidate}\label{fig:repr}
\end{figure}


Seldon allow each event to  different representations ranging from a the full representation which identifies the particular API from a library to a coarse one which only uses the API name. 
Even this approach is sensible we found in practice it could generate many representations and affect the scalability of the constraint solver or even produce to many representations in the produced sinks predictions. 

We follow a different approach. Instead of producing several representations for each program node, we opted for producing only one \emph{canonical} representation. The goal of using canonical representation was: i ) reduce the number of total representations to improve the scalability and  ii) produce many common representations among different projects, which also helped to improve the effect of composing individual projects. 

The ideal of a canonical representation is to produce a representation that is coarse enough to capture many program nodes but detailed enough to not capture too many. The idea is that representation capture typical scenarios like a parameter of a library method, or accessing a member of a object. To find this canonical representation perform an study on the most common representations by essentially producing several representions per node, convert them to patterns (eg., transform \texttt{parameter 0 (member get *)} into \texttt{parameter N (member M *)} and count the number of nodes in a training set matching the patterns. 
We take the top 20 as the patterns of canonical reps. 

%\begin{figure*}
	%	\includegraphics[width=1\textwidth]{figures/TSM-2}
	%	\caption{\tool{} (from a PPT a prepare in February)}        
	%\end{figure*}

